Hypothesis Disparity Regularized Mutual Information Maximization

We propose a hypothesis disparity regularized mutual information maximization~(HDMI) approach to tackle unsupervised hypothesis transfer -- as an effort towards unifying hypothesis transfer learning (HTL) and unsupervised domain adaptation (UDA) -- where the knowledge from a source domain is transferred solely through hypotheses and adapted to the target domain in an unsupervised manner. In contrast to the prevalent HTL and UDA approaches that typically use a single hypothesis, HDMI employs multiple hypotheses to leverage the underlying distributions of the source and target hypotheses. To better utilize the crucial relationship among different hypotheses -- as opposed to unconstrained optimization of each hypothesis independently -- while adapting to the unlabeled target domain through mutual information maximization, HDMI incorporates a hypothesis disparity regularization that coordinates the target hypotheses jointly learn better target representations while preserving more transferable source knowledge with better-calibrated prediction uncertainty. HDMI achieves state-of-the-art adaptation performance on benchmark datasets for UDA in the context of HTL, without the need to access the source data during the adaptation.

==> office31_performance.tex <==
\addtolength{\tabcolsep}{-3pt}
\begin{table*}[!t]
    \centering
    \caption{Target accuracy ($\%$) on Office-31.}
    \begin{adjustbox}{width=\textwidth}
      \begin{tabular}{c*{8}{c}}
        \toprule
        Source & Method & A$\rightarrow$D & A$\rightarrow$W & D$\rightarrow$A & D$\rightarrow$W & W$\rightarrow$A & W$\rightarrow$D & \fcolorbox{gray}{lightgray}{Avg.} \\
        \midrule
        \multirow{5}{*}{\cmark}
        & DAN~\cite{long2015learning} & 78.6 & 80.5 & 63.6 & 97.1 & 62.8 & 99.6 & \fcolorbox{gray}{lightgray}{80.4} \\
        & DANN~\cite{ganin2015unsupervised} & 79.7 & 82.0 & 68.2 & 96.9 & 67.4 & 99.1 & \fcolorbox{gray}{lightgray}{82.2} \\
        % & CDAN+E \\
        & SAFN+ENT~\cite{xu2019larger} & 90.7 & 90.1 & 73.0 & 98.6 & 70.2 & 99.8 & \fcolorbox{gray}{lightgray}{87.1} \\
        & rRevGrad+CAT~\cite{deng2019cluster} & 90.8 & 94.4 & 72.2 & 98.0 & 70.2 & \textbf{100.} & \fcolorbox{gray}{lightgray}{87.6} \\
        & CDAN+BSP~\cite{chen2019transferability} & 93.0 & 93.3 & 73.6 & 98.2 & 72.6 & \textbf{100.} & \fcolorbox{gray}{lightgray}{88.5} \\
        & MDD~\cite{pmlr-v97-zhang19i} & 93.5 & \textbf{94.5} & \textbf{74.6} & 98.4 & 72.2 & \textbf{100.} & \fcolorbox{gray}{lightgray}{88.9} \\
        
        \midrule
        \multirow{8}{*}{\xmark}
        & Source only (single hypothesis) &  79.7 & 75.7 & 61.2 & 96.0 & 59.8 & 98.2 & \fcolorbox{gray}{lightgray}{78.4} \\
        & MI maximization (single hypothesis) & 90.2 & 92.3 & 73.0 & 96.5 & 73.1 & 95.0 & \fcolorbox{gray}{lightgray}{86.7} \\
        & SHOT~\cite{liang2020we} & 92.1 & 89.6 & 74.1 & 98.5 & 73.3 & 99.9 & \fcolorbox{gray}{lightgray}{87.9} \\
        \cmidrule(lr){2-9}
        % & Source only (multiple hypotheses*) & 81.1 & 77.2 & 61.2 & 96.5 & 60.7 & 98.4 & \fcolorbox{gray}{lightgray}{79.2}  \\
        & Source only ensemble (multiple hypotheses*) & \\
        % anchor hypothesis
        % & MI maximization (multiple hypotheses*) & 91.0 & 93.0 & 72.1 & 96.6 & 73.7 & 97.2 & \fcolorbox{gray}{lightgray}{87.3} \\
        & MI ensemble (multiple hypotheses*) & 91.0 & 93.0 & 72.3 & 96.5 & 73.7 & 97.4 & \fcolorbox{gray}{lightgray}{87.3} \\
        
        %%%%%%% 2 classifier version (w=0.3)
        % & HDMI (multiple hypotheses*) & \textbf{94.2} & 94.0 & 73.6 & 98.5 & \textbf{75.5} & 99.8 & \fcolorbox{gray}{lightgray}{\textbf{89.3}} \\
        % & MI ensemble + $L_2$ (multiple hypotheses*) \\
        % & MI ensemble + $L_2$ source (multiple hypotheses*) \\
        %%%%%%% 2 classifier version (w=0.5)
        & HDMI (multiple hypotheses*) & \textbf{94.4} & 94.0 & 73.7 & \textbf{98.9} & \textbf{75.9} & 99.8 & \fcolorbox{gray}{lightgray}{\textbf{89.5}} \\
        & HDMI ensemble (multiple hypotheses*) & \textbf{94.4} & 94.0 & 73.6 & \textbf{98.9} & \textbf{75.9} & 99.8 & \fcolorbox{gray}{lightgray}{89.4} \\
        \bottomrule
        \multicolumn{5}{l}{\footnotesize * Two hypotheses as an illustration. More examples are shown in Table~\ref{tab:robustness}.}
      \end{tabular}
    \end{adjustbox}
    \label{tab:office31}
\end{table*}
\addtolength{\tabcolsep}{3pt}
